Physically Compatible 3D Object Modeling from a Single Image

We present a computational framework that transforms single images into 3D physical objects. The visual geometry of a physical object in an image is determined by three orthogonal attributes: mechanical properties, external forces, and rest-shape geometry. Existing single-view 3D reconstruction methods often overlook this underlying composition, presuming rigidity or neglecting external forces. Consequently, the reconstructed objects fail to withstand real-world physical forces, resulting in instability or undesirable deformation -- diverging from their intended designs as depicted in the image. Our optimization framework addresses this by embedding physical compatibility into the reconstruction process. We explicitly decompose the three physical attributes and link them through static equilibrium, which serves as a hard constraint, ensuring that the optimized physical shapes exhibit desired physical behaviors. Evaluations on a dataset collected from Objaverse demonstrate that our framework consistently enhances the physical realism of 3D models over existing methods. The utility of our framework extends to practical applications in dynamic simulations and 3D printing, where adherence to physical compatibility is paramount.

==> sections/conclusion.tex <==
\section{Conclusion}
In this work, we introduced physical compatibility optimization for reconstructing a physical object from a single image. 
Our method decomposes three orthogonal attributes governing physical behavior: mechanical properties, external forces, and rest-shape geometry. 
Unlike existing methods that often ignore one or more dimensions, our framework holistically considers all three factors, allowing for diverse rest-shape geometries from the same input image by varying object stiffness and external forces. 
We formulate physical compatibility optimization as a constrained optimization problem by integrating static equilibrium as a hard constraint. 
Our approach produces physical objects that match the geometry depicted in the input image under external forces and remain stable under gravity. 
Both quantitative and qualitative evaluations demonstrated improvements in physical compatibility over existing baselines. 
Our method's versatility is evident through its integration with various single-view reconstruction methods and its practical applications in dynamic simulations and 3D printing.

% that incorporates static equilibrium simulation as a hard constraint with the existing single-view 3D reconstruction methods. 
% This integration ensures that the optimized shapes are not only high-quality visual reproductions of the input images 
% but also adhere to real-world physical laws, maintaining structural integrity.
% To validate our framework, 
% we initially demonstrated quantitatively how integrating our method with existing techniques significantly enhances the physical compatibility of the generated shapes compared to those produced by the existing methods alone.
% Furthermore, we evidenced that the shapes optimized through our approach not only closely resemble the visual input but also possess inherent self-supporting capabilities.
% Our methodology provides users with flexibility in generating varied shapes using different materials from the same single input image. 
% The optimized shapes produced are simulation-ready and can seamlessly transition into dynamic simulations. Additionally, these shapes can be realized through 3D printing.
% The 3d-printed shapes closely matches with the input image, 
% expanding the practical utility of existing reconstruction methods in real-world applications.

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}
% pcma: my intro workflow
% 1. 3d content generation grows: (1) one-stage methods (LRM), (2) two-stage methods (mvdream, wonder3d, 0123)
% 2. when applying these 3d content beyond simple visualization, in spite of growing visual quality, these 3d content are not physically ready. As shwon in the top row in Fig1, under real-world physics (e.g. gravity), naively generated 3D objects diverge from their original input images by instability, fragility, or deformation, hindering the scalibity of these methods in interactive applications or real-world deployment.
% 3. to solve this problem, we introduce the concept of physical objects: a 3D object that perceptually matches a given image while inherently conforming to certain physical laws. These physical objects are essential protocols bridging digital content generation and interactive applications due to its visual plausibility and physical realism. As shown in the bottom row in fig1, these physical objects are stable, robust, and high-fidelity 3D replications of the input images under certain physical laws.

The field of single-image 3D shape modeling has experienced significant advancements over the past years, largely propelled by advances in single-view reconstruction techniques. 
These methods,
% encompass a spectrum of approaches, 
ranging from generating multi-view consistent images for per-scene 3D reconstruction~\citep{syncdreamer, wonder3d, zero1to3, realfusion, qian2023magic123, Liu2023-pi}, to employing large reconstruction models (LRMs) 
% that learn general 3D priors for shape reconstruction 
for feedforward inference~\citep{openlrm, triposr, meshlrm, GSLRM, grm, lgm},
have enhanced 
the geometric quality and visual fidelity of the 3D shapes
to 
unprecedented levels.


% Accompanied by the evolution of 3D geometry representation, such as NeRF~\citep{nerf}, NeuS~\citep{NeuS}, triplanes~\citep{triplane}, Gaussian splatting~\citep{3DGS}, surface meshes~\citep{nicolet2021large}, and tet-spheres~\citep{tetsphere}, the geometric quality and visual fidelity of the 3D shapes reconstructed by these methods have reached unprecedented levels.

% 2. when applying these 3d content beyond simple visualization, in spite of growing visual quality, these 3d content are not physically ready. As shwon in the top row in Fig1, under real-world physics (e.g. gravity), naively generated 3D objects diverge from their original input images by instability, fragility, or deformation, hindering the scalibity of these methods in interactive applications or real-world deployment.

% \ma{When applying these 3D objects beyond simple visualization, despite the improvements in visual quality, they are not physically ready for practical use. As shown in the top row of Fig.~\ref{fig:teaser}, when subjected to real-world physics such as gravity, naively generated 3D objects exhibit issues like instability, fragility, or unreasonable deformation. These physical deficiencies cause the 3D objects to diverge from their original input images, thus hindering the scalability and effectiveness of these methods in interactive applications for real-world deployment. For example, these 3D objects will behave counter-physically in physics-based games, leading to unrealistic gameplay experiences. In the animation or film industry, they may perform unpredictably, resulting in scenes that do not meet the desired standards. Additionally, in industrial applications such as 3D printing, these objects may load sub-optimally, causing production inefficiencies and potentially flawed end products.}

However, reconstructing a 3D shape from an image often aims beyond mere visualization: 
These objects find applications across virtual environments such as animation and gaming, as well as in tangible fields like industrial design and fabrication.
Despite their diverse applications, however, a common oversight in many current image-to-3D conversion methods is the lack of consideration of physical principles. 
% In both contexts, 3D objects are embedded within environments governed by rich physical principles; however, these are often overlooked by most existing image-to-3D methods.  
As shown in the top row of Fig.~\ref{fig:teaser}, when subjected to real-world physics such as gravity, naively generated 3D objects exhibit issues like instability and undesirable deformation.
These physical inadequacies lead to a divergence of the 3D models from their intended design, thereby compromising the scalability and effectiveness of these methods in practical scenarios.
% For instance, in physics-based games, such 3D objects might behave in a manner that's not physically plausible. 
% In the realm of manufacturing such as 3D printing, these objects may not be suitable for the fabrication process, resulting in potentially defective products.
% In the animation or film industry, they may act unpredictably, resulting in scenes that fail to meet production standards.
% overlook these underlying physical principles.
% where their behavior is dictated by underlying physical principles.
% , which are often overlooked by existing image-to-3D methods.
% This oversight becomes problematic when the 3D model, even subject to simple physics such as gravity, diverges significantly from the desired appearance prescribed by the input image,
% in its static equilibrium state
% or when its dynamic response to external forces is unrealistic. \gc{We need to add more sentences on the real-world applications. }
% , leading to unpredictable behaviors.
% interactions with the environment.
% \mg{TODO: 1. define "physical object" 2. diff from PhyGaussian/PACNeRF/PhysNeRF 3. explain teaser}
% As shown in xxx.
% \gc{We need a definition of the problem setting. what is the input and output.}
% \mg{the shape in the image is already interacted/entangled with physics}

% 3. to solve this problem, we introduce the concept of physical objects: a 3D object that perceptually matches a given image while inherently conforming to certain physical laws. These physical objects are essential protocols bridging digital content generation and interactive applications due to its visual plausibility and physical realism. As shown in the bottom row in fig1, these physical objects are stable, robust, and high-fidelity 3D replications of the input images under certain physical laws.

% \ma{To solve this problem, we introduce the concept of \emph{physical object}: a 3D object that perceptually matches a given image while inherently conforming to certain physical laws. A physical object is an essential protocol bridging digital content generation and interactive applications due to its visual plausibility and physical stability. Despite the importance, it is constantly overlooked by current literature which either}
{To address this problem, we introduce the concept of \emph{physical objects}: 3D models that not only perceptually match a given image but also inherently conform to certain physical laws. 
% These \emph{physical objects} are crucial protocols that bridge the gap between digital content generation and interactive applications due to their visual plausibility and physical realism. 
As shown in the bottom row of Fig.~\ref{fig:teaser}, these {physical objects} are stable, robust, and high-fidelity replications of the input images, maintaining their integrity under real-world physical laws.
% This ensures they are practical for use in various applications, providing a reliable and realistic experience to 3D practitioners.
}
% This paper focuses on the goal of deriving a \emph{physical object} from a single image.
% We define a physical object as a 3D shape that visually replicates the input image while conforming to physical laws, ensuring both stable and realistic behavior under real-world forces. 
% Fig.~\ref{fig:teaser} showcases examples comparing physical objects with vanilla objects, highlighting \emph{self-support stability} and \emph{equilibrium consistency}. 
% A physical object is inherently stable, maintaining its position without toppling.
% It also aligns closely with the visual appearance of the input image when subjected to external forces such as gravity, thereby maintaining realism through equilibrium consistency.  
The key insight of single-image physical object modeling is that an image is a snapshot capturing an object in a state of static equilibrium, influenced by ongoing physical forces.
This means the object is not just a static form; it reflects a balance of forces at the moment of capture, inherently exhibiting physical behaviors.
Yet, most existing methods often overlook these crucial physical influences when modeling 3D objects from the input image. 
% This means that the depicted object in the image is not merely a static geometry but inherently exhibits physical behaviors.
% Accounting for such existing physical influences is essential in physical object modeling to ensure both self-support stability and equilibrium consistency. 
% Existing research, however, often overlooks this factor; they either separate the shape modeling process by first reconstructing the object’s geometry and then applying physical simulations to this established shape, or rely on dynamic inputs such as videos, which provide a richer temporal context for inferring physical properties.
% This contrast with our challenge of deriving physical objects from a single, static image. 
% Other approaches typically separate the shape modeling process by first reconstructing the object’s geometry and then applying physical simulations to this established shape, thus overlooking the inherent physical forces already present in the initial image.
% Our work diverges by integrating the geometry, material properties, and external forces from the outset, aiming for a holistic model that is both visually and physically congruent with the real world.

% \gc{Give the core idea of our approach: integrate a differentiable physics engine for optimizations. }

\begin{wrapfigure}[17]{r}{0.45\textwidth}
\begin{center}
% \hspace{-1cm}
\includegraphics[width=0.45\textwidth]{figures/3dim.png}
\end{center}
% \caption{Birds}
\end{wrapfigure}
To address this gap, we propose a computational framework termed \emph{physical compatibility} optimization.
This approach integrates static equilibrium physics directly into the modeling of physical objects, optimizing the rest-shape geometry under a \emph{hard constraint} of this physical principle.
At the heart of our approach is the explicit decomposition of the three attributes that govern physical behavior: \emph{mechanical properties} and \emph{external forces}, which are treated as predefined inputs, and \emph{rest-shape geometry}, which is the output.
% The objective of the framework is to ensure that the simulated physical object achieves an equilibrium state that is visually consistent with the input image. 
This decomposition of attributes provides two principal benefits: 
\textbf{1)} It allows for more versatile modeling of physical objects, accommodating variations in object softness and external forces, in contrast to most existing image-to-3D methods that assume objects are rigid solids without external forces;  
\textbf{2)} It enhances the controllability of physical object modeling, allowing for deriving diverse rest-shape geometries by varying the material properties or external forces, which in turn produces diverse dynamic behaviors.

More specifically, we formulate an optimization problem to model a 3D object from an input image.
This optimization is framed as a constrained optimization problem, with rest-shape geometry as the variable. 
The objective is to ensure the modeled physical shape adheres to desired behaviors, such as matching the geometry depicted in the input image under external forces and maintaining stability under gravity.
The constraint is a hard equation derived from static equilibrium simulations.
This ensures that with the specified material properties and external forces, the equilibrium state of the 3D object balances the internal forces -- generated by deformation from the rest shape -- against the external forces.

% \mg{Sora (even 2D generation, no physics, sora a bit more phyiscs), physics (jiang)}
% \mg{rendering first -> stability -> fea}
To comprehensively evaluate physical compatibility, we introduce five evaluation metrics aimed at assessing the physical realism and reliability of the modeled 3D objects under simulation. 
These metrics include rendered loss between the modeled object and the input image, stability under gravity, as well as measures from finite element analysis, such as integrity and structural robustness.
Our framework's versatility is demonstrated through its integration with five distinct single-view reconstruction methods, each employing unique geometry representations. 
Results on an evaluation dataset collected from Objaverse~\citep{objaverse}, consisting of $100$ shapes, demonstrate that our framework consistently produces 3D objects with enhanced physical compatibility. 
Furthermore, we demonstrate the practical utility of our framework through applications in 3D printing fabrication and dynamics simulations.

% The resulting model not only conforms to physical laws, such as gravity and stability, but is also 

% optimally configured for immediate application in downstream processes, such as 3D printing and physics-informed video generation.

% By embedding physical realism into the 3D modeling pipeline, this paper endeavors to harmonize the digital and physical realms, significantly enhancing the functional reliability and application scope of 3D models derived from single images.



==> sections/introduction.v2.tex <==
\section{Introduction}
\label{sec:intro}
The field of single-image 3D shape modeling has experienced significant advancements over the past years, largely propelled by advances in single-view reconstruction techniques. 
These methods,
ranging from generating multi-view consistent images for per-scene 3D reconstruction~\citep{syncdreamer, wonder3d, zero1to3, realfusion, qian2023magic123, Liu2023-pi}, to employing large reconstruction models (LRMs) 
for feedforward inference~\citep{openlrm, triposr, meshlrm, GSLRM, grm, lgm},
have enhanced the geometric quality and visual fidelity of the 3D shapes to 
unprecedented levels.

However, reconstructing a 3D shape from an image often aims to be beyond a mere visualization.
These generated objects find applications in virtual environments 
such as filming and gaming, 
as well as in tangible fields like industrial design and engineering.
Despite their diverse applications, 
a common oversight in many current single-view reconstruction methods is the negligence of physical principles.
As shown in the top row of Fig.~\ref{fig:teaser}, 
when subjected to real-world physics such as gravity, 
these 3D objects 
produced from these techniques 
exhibit issues such as instability and undesired deformation, diverging from their depiction in the input images.
Such inconsistency can significantly undermine the practical utility of the models, as they fail to meet the functional and aesthetic expectations set by the original image.
The underlying reason is that an input image is not merely a visual representation;
it captures a physical snapshot of the object in a state of static equilibrium, under the influence of real-world forces.
% Thus, the image captures a momentary equilibrium of forces, 
% inherently implying physical behavior. 
% Nevertheless, the majority of 
Current methods tend to merely replicate these static shapes without considering the inherent physical contexts, which are crucial to ensure the reconstructed model accurately reflects the static physical behavior of the original object.
% altered deformation under real-world physics.
This oversight leads to significant discrepancies between the reconstructed models and their intended designs, thereby limiting their practical applicability.
% as it fails to meet the functional and aesthetic expectations set by the original image.
% of these methods.

\begin{wrapfigure}[14]{r}{0.37\textwidth}
	\begin{center}
		% \hspace{-1cm}
		\includegraphics[width=0.37\textwidth]{figures/3dim.pdf}
	\end{center}
	% \caption{Birds}
\end{wrapfigure}

To bridge this gap, we propose a method to reconstruct a \emph{physical object} from a single image, using a computational framework we call \emph{physical compatibility} optimization.
% In our context, a 
A physical object refers to a reconstructed shape that not only mirrors the object's static equilibrium state depicted in the image but also maintains stability under real-world physical conditions. 
Our approach integrates static equilibrium physics directly into the modeling of 3D objects, 
% optimizing the rest-shape geometry under 
enforcing it as a \emph{hard constraint}.
% of this physical principle.
These optimized {physical objects} are stable, robust, and high-fidelity replicas inferred from the input images, 
% maintaining their integrity under real-world physical laws,
as shown in the bottom row of Fig.~\ref{fig:teaser}.
At the heart of our approach is the explicit decomposition of the three attributes that govern physical behavior: \emph{mechanical properties}, \emph{external forces}, and \emph{rest-shape geometry}.
These three attributes are orthogonal dimensions that fully determine the static equilibrium state of an object, as shown in the inset figure.
In this context, existing methods only treat objects as rigid materials or neglect external forces, thereby ignoring at least one dimension of this decomposition.
Our framework holistically considers all three factors by taking
% Altering each of them leads to different shapes under physics (see inset figure).
% In our framework, we  
{mechanical properties} and {external forces}
as pre-defined inputs, and {rest-shape geometry} as the output.
% As a result, 
% it
This allows for more diverse rest-shape geometries even from the same input image by varying object stiffness and external forces.
% in contrast to most existing image-to-3D methods that assume objects are rigid solids without external forces.

%\textbf{2)} It enhances the controllability of physical object modeling, allowing for deriving diverse rest-shape geometries by varying the material properties or external forces, which in turn produces diverse dynamic behaviors.

More specifically, 
% we formulate an optimization problem to model a 3D object from an input image.
we frame physical compatibility optimization as a constrained optimization problem, with rest-shape geometry as the variable. 
The objective is for the modeled physical object to exhibit desired behaviors, such as matching the geometry depicted in the input image under external forces and maintaining stability under gravity.
The constraint is the equation of static equilibrium simulation, ensuring that during optimization, the physical object remains in the equilibrium state, with internal forces generated by deformation from the rest shape balancing the external forces.
% with the specified material properties and external forces, 
% the equilibrium state of the 3D object balances the internal forces -- generated by deformation from the rest shape -- against the external forces.

%A realistic 3D object should equip physical properties and conform to physical laws, which we denote them \emph{physical objects}.
%As shown in the bottom row of Fig.~\ref{fig:teaser}, 

% \mg{Sora (even 2D generation, no physics, sora a bit more phyiscs), physics (jiang)}
% \mg{rendering first -> stability -> fea}
For evaluation, we introduce five metrics designed to comprehensively assess the physical compatibility of the modeled 3D objects under simulation. 
% To comprehensively evaluate the physical compatibility, we introduce five evaluation metrics designed to assess the physical realism and reliability of the modeled 3D objects under simulation. 
These metrics include image loss between the rendered image of the modeled physical object and the input image, stability under gravity, as well as measures from finite element analysis, such as integrity and structural robustness.
Our framework's versatility is demonstrated by its integration with five distinct single-view reconstruction methods, each employing unique geometry representations.
Results on a dataset collected from Objaverse~\citep{objaverse}, consisting of $100$ shapes, show that our framework consistently produces 3D objects with enhanced physical compatibility. 
Furthermore, we demonstrate the practical utility of our framework through applications in dynamic simulations and 3D printing fabrication.

% The resulting model not only conforms to physical laws, such as gravity and stability, but is also 

% optimally configured for immediate application in downstream processes, such as 3D printing and physics-informed video generation.

% By embedding physical realism into the 3D modeling pipeline, this paper endeavors to harmonize the digital and physical realms, significantly enhancing the functional reliability and application scope of 3D models derived from single images.



==> sections/related_work.tex <==
% \section{Related Work}
\paragraph{Related work.}
Our method is mainly related to: \textbf{1)} single-view 3D reconstruction, where our work emphasizes the integration of physical modeling into the reconstruction process; \textbf{2)} physically based 3D modeling, where we incorporate physical principles as hard constraints within the reconstruction process; and \textbf{3)} fabrication-aware shape design, where our work directly constructs physical objects from a single input image rather than relying on manual creation of the initial geometry.
A comprehensive discussion of related work is provided in Appendix~\ref{app:related_work}.

